ECNN: A Low-complex, Adjustable CNN for Industrial Pump Monitoring Using Vibration Data

Industrial pumps are essential components in various sectors, such as manufacturing, energy production, and water treatment, where their failures can cause significant financial and safety risks. Anomaly detection can be used to reduce those risks and increase reliability. In this work, we propose a novel enhanced convolutional neural network (ECNN) to predict the failure of an industrial pump based on the vibration data captured by an acceleration sensor. The convolutional neural network (CNN) is designed with a focus on low complexity to enable its implementation on edge devices with limited computational resources. Therefore, a detailed design space exploration is performed to find a topology satisfying the trade-off between complexity and accuracy. Moreover, to allow for adaptation to unknown pumps, our algorithm features a pump-specific parameter that can be determined by a small set of normal data samples. Finally, we combine the ECNN with a threshold approach to further increase the performance and satisfy the application requirements. As a result, our combined approach significantly outperforms a traditional statistical approach and a classical CNN in terms of accuracy. To summarize, this work provides a novel, low-complex, CNN-based algorithm that is enhanced by classical methods to offer high accuracy for anomaly detection of industrial pumps.

==> makros_own.tex <==


\newcommand{\ffw}{0.7\columnwidth} %{0.285\columnwidth}
\newcommand{\ffh}{0.56\columnwidth} %{0.23\columnwidth}



%\DeclareMathOperator{\fft}{\mathcal{F}}
%\DeclareMathOperator{\ifft}{\mathcal{F}^{-1}}
\newcommand{\fft}[1]{\mathcal{F}\mleft\{#1\mright\}}
\newcommand{\ifft}[1]{\mathcal{F}^{-1}\mleft\{#1\mright\}}

\DeclareMathOperator{\E}{\mathbb{E}}
\DeclareMathOperator{\Eq}{\mathbb{E}_{q_{\bm{\Phi}}\mlr{\bm{X}\mid \bm{Y}}}}

\newcommand{\elr}{\epsilon_{\mathrm{lr}}} % learning rate
\newcommand{\Nos}{N_{\mathrm{os}}}    % oversampling factor
\newcommand{\Nti}{N_{\mathrm{TI}}}    % number of training iterations
\newcommand{\Nb}{N_{\mathrm{b}}}    % batch-size
\newcommand{\Nd}{N_{\mathrm{d}}}    % number of discr. updates per TI
\newcommand{\Nch}{N_{\mathrm{ch}}}    % number of channels (in CNN)
\newcommand{\Nparam}{N_{\mathrm{param}}}    % number of channels (in CNN)
\newcommand{\Fma}{F_{\mathrm{ma}}}    % filter length of MA (results)
\newcommand{\varN}{\sigma^2_{\mathrm{n}}} % noise variance
\newcommand{\varRefi}{\sigma_\mathrm{ref}^{2}\mlr{i}} % variance of added noise to reference
\newcommand{\Lf}{L_{\mathrm{fiber}}} % fibre length
\newcommand{\adB}{\alpha_{\mathrm{dB}}} % attenuation

%\newcommand{\snr}{\mathrm{SNR}} % fibre length



\newcommand{\lr}[1]{\left(#1\right)}
\newcommand{\mlr}[1]{\mleft(#1\mright)}
\newcommand{\mlrb}[1]{\mleft\{#1\mright\}}

\DeclareMathSymbol{\mlq}{\mathord}{operators}{``}
\DeclareMathSymbol{\mrq}{\mathord}{operators}{`'}

\newcommand{\normDis}[2]{\mathcal{N}\mlr{#1,\,#2}}
\newcommand{\multiNormDis}[3]{\mathcal{N}_{#3}\mlr{#1,\,#2}}
\newcommand{\uniDisN}[2]{\mathcal{U}\mlr{#1,\,#2}}
\newcommand{\multiUniDis}[3]{\mathcal{U}_{#3}\mlr{#1,\,#2}}


% simple implication within math or text
\def\thus{\relax
	\ifmmode
	\implies
	\else
	$\implies$
	\fi}


% Pointing finger for noting important things
\newcommand{\mind}{ \hfill { \textbf{\textcolor{KITred}{\bf \HandLeft} } } }


% colored small box representing end of a proof
\def\endofproof{
	\ifmmode
		\text{\hfill} \textcolor{KITgreen}{\rule{2mm}{2mm}}
	\else
		$\hfill \textcolor{KITgreen}{\rule{2mm}{2mm}}$
	\fi}



%%%%%%%%%%%%%%%%%
% Basic math
%%%%%%%%%%%%%%%%%

% definition sign
\def\defl{:=}

% j and differential calc
\def\j{{\mathrm{j}}}
\def \dd{\, {\mathrm{d}}}

% Real part
\def\real{{\mathrm{Re}}}
\def\imag{{\mathrm{Im}}}

\def\I{{\mathrm{I}}}
\def\Q{{\mathrm{Q}}}

\def\TE{{\mathrm{TE}}}
\def\TM{{\mathrm{TM}}}

\def\H{{\mathrm{H}}}

% Vector notataion
\newcommand\vek[1]{{\bm{#1}}}

% sinc and rect
\newcommand\sinc{{\mathrm{sinc}}}
\newcommand\rect{{\mathrm{rect}}}


% Galois
\def\F{{\mathbb{F}}}


% fields
\def\rz{\ifmmode{\mathbb{R}}%
    \else{\hbox{$\mathbb{R}$}}\fi} 
\def\nz{\ifmmode{\mathbb{N}}%
    \else{\hbox{$\mathbb{N}$}}\fi} 
\def\gz{\ifmmode{\mathbb{Z}}%
   \else{\hbox{$\mathbb{Z}$}}\fi} 
\def\cz{\ifmmode{\mathbb{C}}
    \else{\hbox{$\mathbb{C}$}}\fi}%
\def\qz{\ifmmode{\mathbb{Q}}%
    \else{\hbox{$\mathbb{Q}$}}\fi}%   
\def\K{\ifmmode{\mathbb{K}}%
    \else{\hbox{$\mathbb{K}$}}\fi}%  


% Sets as caligraphic letters
\def\setS{{\mathcal{S}}}
\def\setP{{\mathcal{P}}}
\def\setX{{\mathcal{X}}}
\def\setY{{\mathcal{Y}}}
\def\setZ{{\mathcal{Z}}}
\def\setC{{\mathcal{C}}}
\def\setB{{\mathcal{B}}}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Probability theory
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Er{\ifmmode{\mathbb{E}}%
    \else{\hbox{$\mathbb{E}$}}\fi}%  
    
\def\V{
	\ifmmode
	{\mathrm{V}}
	\else
	${\mathrm{V}}$
	\fi}    


\def\PO{\mathcal{P}(\Omega)}
\def\sigalg{\mathcal{B}}

\def\NO{N_{\Omega}}
	
% random variables
%\newcommand\rv[1]{{\mathsf{#1}}}
\newcommand\rv[1]{{\uppercase{#1}}}

\def\rvX{\rv{x}}
\def\rvY{\rv{y}}
\def\rvZ{\rv{z}}






%%%%%%%%%%%%%%%%%
% Communications, system theory, and transforms
%%%%%%%%%%%%%%%%%


% Bandpass as Index
\def\bp{{\mathrm{BP}}}


% transform as symbol
\usepackage{trfsigns}

\def\transform{\; \laplace \;}
\def\Transform{\; \Laplace \;}

\newcommand{\vTransform}[1][]{\mbox{\setlength{\unitlength}{0.1em}%
		\begin{picture}(10,20)%
		\put(3,2){\circle{4}}%
		\put(3,4){\line(0,1){12}}%
		\put(3,18){\circle*{4}}%
		\put(10,7){#1}
		\end{picture}%
	}%
}%

\newcommand{\vtransform}[1][]{\mbox{\setlength{\unitlength}{0.1em}%
		\begin{picture}(10,20)%
		\put(3,2){\circle*{4}}%
		\put(3,4){\line(0,1){12}}%
		\put(3,18){\circle{4}}%
		\put(10,7){#1}
		\end{picture}%
	}%
}%     


% Hz and seconds
\newcommand\uHz{\mu{\,\mathrm{Hz}}}
\newcommand\us{{\mu\,\mathrm{s}}}	

% index for indicating sample time
\newcommand\samp{{\mathrm{s}}}

% samples per symbol
\newcommand\sps{{\text{sps}}}

% command for SNR as sans-serif
\newcommand\snr{{\mathsf{SNR}}}

\newcommand\ser{{\mathsf{SER}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Boxes and stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% Command for aligning itemize when using columns; --> add "\AdjustMargins" after \begin{frame}...
\makeatletter
\newcommand*{\AdjustMargins}{%
    \setlength{\beamer@rightmargin}{0em}%
    \setlength{\beamer@leftmargin}{0em}%
}
\makeatother





\newcommand{\myfn}[1]{\footnote{\scriptsize {#1}}}

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}


\newcommand\nomarkfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{\scriptsize #1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}



%% \highlight[<colour>]{<stuff>}
%\newcommand{\hi}[2][KITyellow]{
%	\ifmmode
%	{
%		\begin{switch}{#1}
%		\case{white}
%			{
%			\mathchoice%
%			  {\colorbox{#1}{$\displaystyle#2$}}%
%			  {\colorbox{#1}{$\textstyle#2$}}%
%			  {\colorbox{#1}{$\scriptstyle#2$}}%
%			  {\colorbox{#1}{$\scriptscriptstyle#2$}}
%			}
%		\case{KITyellow}
%			{
%				 \mathchoice%
%				  {\colorbox{#1}{$\displaystyle#2$}}%
%				  {\colorbox{#1}{$\textstyle#2$}}%
%				  {\colorbox{#1}{$\scriptstyle#2$}}%
%				  {\colorbox{#1}{$\scriptscriptstyle#2$}}
%			}%
%		\case{KITorange}
%			{
%				 \mathchoice%
%				  {\colorbox{#1}{$\displaystyle#2$}}%
%				  {\colorbox{#1}{$\textstyle#2$}}%
%				  {\colorbox{#1}{$\scriptstyle#2$}}%
%				  {\colorbox{#1}{$\scriptscriptstyle#2$}}
%			}%			
%		\case{KITred}
%			{
%				 \mathchoice%
%				  {\colorbox{#1}{\textcolor{white}{$\displaystyle#2$}}}%
%				  {\colorbox{#1}{\textcolor{white}{$\textstyle#2$}}}
%				  {\colorbox{#1}{\textcolor{white}{$\scriptstyle#2$}}}
%				  {\colorbox{#1}{\textcolor{white}{$\scriptscriptstyle#2$}}}
%			}%	
%		\case{KITblue}
%			{
%				 \mathchoice%
%				  {\colorbox{#1}{\textcolor{white}{$\displaystyle#2$}}}%
%				  {\colorbox{#1}{\textcolor{white}{$\textstyle#2$}}}
%				  {\colorbox{#1}{\textcolor{white}{$\scriptstyle#2$}}}
%				  {\colorbox{#1}{\textcolor{white}{$\scriptscriptstyle#2$}}}
%			}%
%		\case{KITgreen}
%			{
%				 \mathchoice%
%				  {\colorbox{#1}{\textcolor{white}{$\displaystyle#2$}}}%
%				  {\colorbox{#1}{\textcolor{white}{$\textstyle#2$}}}
%				  {\colorbox{#1}{\textcolor{white}{$\scriptstyle#2$}}}
%				  {\colorbox{#1}{\textcolor{white}{$\scriptscriptstyle#2$}}}
%			}%	
%		\case{KITpurple}
%			{
%				 \mathchoice%
%				  {\colorbox{#1}{\textcolor{white}{$\displaystyle#2$}}}%
%				  {\colorbox{#1}{\textcolor{white}{$\textstyle#2$}}}
%				  {\colorbox{#1}{\textcolor{white}{$\scriptstyle#2$}}}
%				  {\colorbox{#1}{\textcolor{white}{$\scriptscriptstyle#2$}}}
%			}%	
%		\case{KITcyan}
%			{
%				 \mathchoice%
%				  {\colorbox{#1}{\textcolor{white}{$\displaystyle#2$}}}%
%				  {\colorbox{#1}{\textcolor{white}{$\textstyle#2$}}}
%				  {\colorbox{#1}{\textcolor{white}{$\scriptstyle#2$}}}
%				  {\colorbox{#1}{\textcolor{white}{$\scriptscriptstyle#2$}}}
%			}%												
%		\end{switch}
%	}
%	\else	
%	{
%	\textcolor{#1}{\textbf #2}
%	}
%	\fi
%	}


% \highlight[<colour>]{<stuff>}
\newcommand{\hi}[2][KITyellow]{
	\ifmmode
	{
		%\tikz[baseline]{\node[fill=#1!50,anchor=base ]{$#2$};}
		 \mathchoice%		
%			{\tikz[baseline]{\node[fill=#1!50,anchor=base ]{$\displaystyle#2$};} }
%			{\tikz[baseline]{\node[fill=#1!50,anchor=base ]{$\textstyle#2$};} }
%			{\tikz[baseline]{\node[fill=#1!50,anchor=base ]{$\scriptstyle#2$};} }
%			{\tikz[baseline]{\node[fill=#1!50,anchor=base ]{$\scriptscriptstyle#2$};} }
			{\colorbox{#1!50}{\textcolor{black}{$\displaystyle#2$}}}%
			{\colorbox{#1!50}{\textcolor{black}{$\textstyle#2$}}}
			{\colorbox{#1!50}{\textcolor{black}{$\scriptstyle#2$}}}
			{\colorbox{#1!50}{\textcolor{black}{$\scriptscriptstyle#2$}}}
	}
	\else
	{
		%\textcolor{#1}{\textbf{#2}}
		{\colorbox{#1!50}{\textcolor{black}{#2}}}
	}
	\fi
	}

	
% Kommando um Hin- und Herschieben zu verhinden
\newcommand{\white}[1]{\textcolor{white}{{#1}}}


% footnotetext that is switched off on the slides given by the first argument
\newcommand{\footnotetextoff}[2]{\alt<#1>{\let\thefootnote\relax\footnotetext{~}}{\footnotetext{\scriptsize #2}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Pages notes and reference
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%
% KIT-Farben
%
\definecolor{kit-green100}{rgb}{0,.59,.51}
\definecolor{kit-green70}{rgb}{.3,.71,.65}
\definecolor{kit-green50}{rgb}{.50,.79,.75}
\definecolor{kit-green30}{rgb}{.69,.87,.85}
\definecolor{kit-green15}{rgb}{.85,.93,.93}
\definecolor{KITgreen}{rgb}{0,.59,.51}

\definecolor{KITpalegreen}{RGB}{130,190,60}
\colorlet{kit-maigreen100}{KITpalegreen}
\colorlet{kit-maigreen70}{KITpalegreen!70}
\colorlet{kit-maigreen50}{KITpalegreen!50}
\colorlet{kit-maigreen30}{KITpalegreen!30}
\colorlet{kit-maigreen15}{KITpalegreen!15}

\definecolor{KITblue}{rgb}{.27,.39,.66}
\definecolor{kit-blue100}{rgb}{.27,.39,.67}
\definecolor{kit-blue70}{rgb}{.49,.57,.76}
\definecolor{kit-blue50}{rgb}{.64,.69,.83}
\definecolor{kit-blue30}{rgb}{.78,.82,.9}
\definecolor{kit-blue15}{rgb}{.89,.91,.95}

\definecolor{KITyellow}{rgb}{.98,.89,0}
\definecolor{kit-yellow100}{cmyk}{0,.05,1,0}
\definecolor{kit-yellow70}{cmyk}{0,.035,.7,0}
\definecolor{kit-yellow50}{cmyk}{0,.025,.5,0}
\definecolor{kit-yellow30}{cmyk}{0,.015,.3,0}
\definecolor{kit-yellow15}{cmyk}{0,.0075,.15,0}

\definecolor{KITorange}{rgb}{.87,.60,.10}
\definecolor{kit-orange100}{cmyk}{0,.45,1,0}
\definecolor{kit-orange70}{cmyk}{0,.315,.7,0}
\definecolor{kit-orange50}{cmyk}{0,.225,.5,0}
\definecolor{kit-orange30}{cmyk}{0,.135,.3,0}
\definecolor{kit-orange15}{cmyk}{0,.0675,.15,0}

\definecolor{KITred}{rgb}{.63,.13,.13}
\definecolor{kit-red100}{cmyk}{.25,1,1,0}
\definecolor{kit-red70}{cmyk}{.175,.7,.7,0}
\definecolor{kit-red50}{cmyk}{.125,.5,.5,0}
\definecolor{kit-red30}{cmyk}{.075,.3,.3,0}
\definecolor{kit-red15}{cmyk}{.0375,.15,.15,0}

\definecolor{KITlilac}{RGB}{160,0,120}
\colorlet{kit-lila100}{KITlilac}
\colorlet{kit-lila70}{KITlilac!70}
\colorlet{kit-lila50}{KITlilac!50}
\colorlet{kit-lila30}{KITlilac!30}
\colorlet{kit-lila15}{KITlilac!15}

\definecolor{KITcyanblue}{RGB}{80,170,230}
\colorlet{kit-cyanblue100}{KITcyanblue}
\colorlet{kit-cyanblue70}{KITcyanblue!70}
\colorlet{kit-cyanblue50}{KITcyanblue!50}
\colorlet{kit-cyanblue30}{KITcyanblue!30}
\colorlet{kit-cyanblue15}{KITcyanblue!15}


% %\definecolor{ALUColor1}{rgb}{0,0.4470,0.7410}
% %\definecolor{ALUColor2}{rgb}{0.8500,0.3250,0.0980}
% \definecolor{ALUColor3}{rgb}{0.9290,0.6940,0.1250}
% %\definecolor{ALUColor4}{rgb}{0.4940,0.1840,0.5560}
% %\definecolor{ALUColor5}{rgb}{0.4660,0.6740,0.1880}
% % colorbrewer 6-class Set1 (qualitative)
% \definecolor{ALUColor1}{RGB}{77,175,74} % colorbrewer 3 (CMA)
% \definecolor{ALUColor2}{RGB}{228,26,28} % colorbrewer 1 (VAE-LE)
% %\definecolor{ALUColor3}{RGB}{77,175,74}
% \definecolor{ALUColor4}{RGB}{55,126,184} % colorbrewer 2 (VAE-NN)
% \definecolor{ALUColor6}{RGB}{152,78,163}

% \definecolor{ALUColor5}{RGB}{255,127,0}
% \definecolor{ALUColor7}{rgb}{0.6350,0.0780,0.1840}

% \definecolor{ALUColor1_70}{rgb}{0,0.3129,0.5187}
% \definecolor{ALUColor2_70}{rgb}{0.5950,0.2275,0.0686}
% %\definecolor{ALUColor2_light}{rgb}{1,0.3823529411,0.115294117624}
% \definecolor{ALUColor2_light}{RGB}{226,97,99}

% \definecolor{ALUColor1_dark}{RGB}{14, 108, 1} 
% \definecolor{ALUColor1_light}{RGB}{0,104,55} 
% \definecolor{ALUColor1_blue}{RGB}{11, 196, 86} 

% % colorbrewer2.0 7-class Set3 (qualitative) --- too bright?
% \definecolor{ALUColor4}{RGB}{141,211,199}   % ganLin
% \definecolor{ALUColor3}{RGB}{255,255,179}   % supLin
% \definecolor{ALUColor7}{RGB}{190,186,218}   % woEq
% \definecolor{ALUColor2}{RGB}{251,128,114}   % sup
% \definecolor{ALUColor5}{RGB}{128,177,211}   % lms
% \definecolor{ALUColor6}{RGB}{253,180,98}    % VNLE
% \definecolor{ALUColor1}{RGB}{179,222,105}   % gan

% % colorbrewer2.0: mix of 5-class RdYlGn and Spectral (diverging)
% \definecolor{ALUColor4}{RGB}{43,131,186}   % ganLin
% \definecolor{ALUColor3}{RGB}{255,255,191}   % supLin
% \definecolor{ALUColor7}{RGB}{166,217,106}   % woEq
% \definecolor{ALUColor2}{RGB}{253,174,97}   % sup
% \definecolor{ALUColor5}{RGB}{171,221,164}   % lms
% \definecolor{ALUColor6}{RGB}{26,150,65}    % VNLE
% \definecolor{ALUColor1}{RGB}{215,25,28}   % gan

% % colorbrewer2.0: 7-class paired (qualitative)
% \definecolor{ALUColor4}{RGB}{251,154,153}   % ganLin
% \definecolor{ALUColor3}{RGB}{166,206,227}   % supLin
% \definecolor{ALUColor7}{RGB}{253,191,111}   % woEq
% \definecolor{ALUColor2}{RGB}{31,120,180}   % sup
% \definecolor{ALUColor5}{RGB}{51,160,44}   % lms
% \definecolor{ALUColor6}{RGB}{178,223,138}    % VNLE
% \definecolor{ALUColor1}{RGB}{227,26,28}   % gan

% colorbrewer2.0: 9-class Set1 (qualitative)
\definecolor{ALUColor4}{RGB}{255,127,0}   % ganLin
\definecolor{ALUColor3}{RGB}{77,175,74}   % supLin
\definecolor{ALUColor7}{RGB}{153,153,153}   % woEq
\definecolor{ALUColor2}{RGB}{55,126,184}   % sup
\definecolor{ALUColor5}{RGB}{152,78,163}   % lms
\definecolor{ALUColor6}{RGB}{166,86,40}    % VNLE
\definecolor{ALUColor1}{RGB}{228,26,28}   % gan

% colorbrewer2.0: 4-class OrRd (sequential)
\definecolor{ALUColor1v}{RGB}{253,204,138}   % ganLin
\definecolor{ALUColor2v}{RGB}{252,141,89}   % supLin
\definecolor{ALUColor3v}{RGB}{215,48,31}   % woEq

